Efficiently Learning Mixtures of Mallows Models

Mixtures of Mallows models are a popular generative model for ranking data coming from a heterogeneous population. They have a variety of applications including social choice, recommendation systems and natural language processing. Here we give the first polynomial time algorithm for provably learning the parameters of a mixture of Mallows models with any constant number of components. Prior to our work, only the two component case had been settled. Our analysis revolves around a determinantal identity of Zagier which was proven in the context of mathematical physics, which we use to show polynomial identifiability and ultimately to construct test functions to peel off one component at a time. To complement our upper bounds, we show information-theoretic lower bounds on the sample complexity as well as lower bounds against restricted families of algorithms that make only local queries. Together, these results demonstrate various impediments to improving the dependence on the number of components. They also motivate the study of learning mixtures of Mallows models from the perspective of beyond worst-case analysis. In this direction, we show that when the scaling parameters of the Mallows models have separation, there are much faster learning algorithms.

==> extras.tex <==
Now we are ready to complete the proof of the main result.  It suffices to show how given a candidate mixture, decide whether it is component-wise $\theta$-close to the true mixture.

\begin{theorem}
Assume we have a mixture of $k$ Mallows models $M_1(\phi_1, \pi_1), \cdots M_k(\phi_k, \pi_k)$ on $n > 10k^2$ elements that is $(\mu,\alpha)$-distinct.  Then by taking $\big( \frac{nk \log \frac{1}{\delta}}{\epsilon \theta \alpha} \big)^{(10k)^{10k}}$ samples from the mixture, there exists a $poly(n,\frac{1}{\epsilon},\frac{1}{\alpha},\frac{1}{\theta}, \log \frac{1}{\delta})$ algorithm for fixed $k$ that learns all of the $\pi_i$ and $w_i,\phi_i$ to within $\theta$ with probability $1-\delta$.  
\end{theorem}
\begin{proof} Let $\gamma = \big( \frac{\epsilon \theta \alpha}{nk \log \frac{1}{\delta}} \big)^{(10k)^{10k}}$.  First, if there is any $\phi_i < \frac{1}{2n}$, then the probability of generating $\pi_i$ is at least $\frac{w_i}{2} \geq \frac{\alpha}{2}$ (this is immediate from the proof of Lemma \ref{TVbound}).  Thus, we sample from the distribution and take all permutations that appear with probability at least $\frac{\alpha}{4}$.  There are at most $\frac{4}{\alpha}$ such samples and with $1- \frac{\delta}{3}$ probability, for each $\phi_i \leq \frac{1}{2n}$, $\pi_i$ is included in this set.  For each of the permutations in this set, consider  the $(\frac{1}{\gamma})^2$ possibilities for the weight and scaling parameter where we use a $\gamma$-grid.  This gives a polynomially sized list say $L$.
\\\\
Now sample from the mixture to construct an estimate of $v = w_1v_c(M_1) + \cdots + w_kv_c(M_k)$.  We can ensure $||v-(w_1v_c(M_1) + \cdots + w_kv_c(M_k))||_{L^1} < \frac{1}{k^2}\bigg(\frac{\epsilon\alpha}{2nk} \bigg)^{60k^4}$ with probability at least $1- \frac{\delta}{3}$.  Now guess a set of at most $k$ elements from $L$ and subtract their corresponding vectors from $v$.  WLOG $\phi_1, \phi_2, \cdots, \phi_j < \frac{1}{2n} \leq \phi_{j+1}, \cdots ,\phi_k$.  If the components we guess say $(w_1', M_1'(\phi_1', \pi_1')), \cdots (w_j', M_j'(\phi_j', \pi_j'))$ satisfy $|w_a - w_a'| < \gamma, |\phi_a - \phi_a'| < \gamma, \pi_a' = \pi_a$ for $1 \leq a \leq j$ then we claim 
\[
||(v-(w_1'v_c(M_1') + \cdots +w_j'v_c(M_j'))-(w_{j+1}v_c(M_{j+1})+ \cdots w_kv_c(M_k))||_{L^1} \leq \frac{1}{k}\bigg( \frac{\epsilon\alpha}{2nk} \bigg)^{60k^4}
\]
This is true since using  Lemma \ref{TVbound} we get $||w_a'v_c(M_a')-w_av_c(M_a)||_{L^1} \leq n^c(10n^3\gamma)^{0.5}$.
\\\\
Thus assuming we guess all of the components with small scaling parameter correctly (which we can accomplish in polynomially many tries), we can apply Corollary \ref{learn2} to output a polynomially sized set which must include all of the true components to within $\gamma$.
\\\\
To summarize what we have shown so far, we can output a list of polynomially many possible $k$-tuples of components one of which must be pairwise $\gamma$-close to the true set of components (just enumerate over all guesses for the $j$ initial components and all $k-j$-tuples from the set above).  It remains to verify that only a set of components pairwise close to the true $k$-tuple can have $||(w_1'v_c(M_1') + \cdots +w_j'v_c(M_j'))-(w_1v_c(M_1) + \cdots + w_kv_c(M_k))||_{L^1}$ sufficiently small.  First, we will eliminate candidates in which some two components have the same base permutation and the scaling parameters within $\frac{\epsilon}{10}$.  We will also eliminate candidates with a scaling parameter more than $1-\frac{\epsilon}{2}$ or mixing weight less than $\frac{\alpha}{2}$.  Note by the way we chose $\gamma$, the $k$-tuples that are $\gamma$-close to the true components will not be eliminated.  We claim that all of the $k$-tuples remaining will have components $\frac{\epsilon}{40}$-separated in total-variation distance.  To see this, for any two components with different base permutations, we use Claim \ref{simple}.  Otherwise, pick two elements that are consecutive in the (shared) base permutation.  Say the scaling parameters are $\phi_i,\phi_j$.  The probability that the two elements occur in order in a sample from the first Mallows model is $\frac{1}{1+\phi_i}$ while for the second Mallows model the probability is $\frac{1}{1+\phi_j}$.  The difference of these quantities is at least $\frac{|\phi_i - \phi_j|}{4}$ giving us the lower bound on the total variation distance.
\\\\

Now the verification step follows from Claim \ref{localIdentifiability}.  Since we set $\gamma \leq  \big( \frac{\epsilon \theta \alpha}{nk} \big)^{(10k)^{10k}}$, we know there exists a hypothesis in our set such that 
\[
||(w_1v_c(M_1) + \cdots + w_kv_c(M_k)) - (w_1'v_c(M_1') + \cdots + w_k'v_c(M_k'))||_{L^1} \leq  \big( \frac{\epsilon \theta \alpha}{nk} \big)^{(10k)^{9k}}
\]
We also know that if the difference above is at most $\big( \frac{\epsilon \theta \alpha}{nk} \big)^{(10k)^{7k}}$ then our hypothesis is satisfactory (since both mixtures are $(\epsilon, \alpha)$-distinct).  We can approximate $(w_1'v_c(M_1') + \cdots + w_k'v_c(M_k'))$ for each of our hypothetical $k$-tuples of components by simulating sampling from the hypothetical mixture (this can be done efficiently as shown in Section $2$ of \cite{Pairwise}).  We can also approximate $v$ by sampling from the real mixture.
\\\\
With failure probability at most $\frac{\delta}{3}$, if we take $\big( \frac{nk \log \frac{1}{\delta}}{\epsilon \theta \alpha} \big)^{(10k)^{10k}}$ samples for our approximations, one of our candidate $k$-tuples will satisfy $||v-(w_1'v_c(M_1') + \cdots + w_k'v_c(M_k'))||_{L^1} \leq \big( \frac{\epsilon \theta \alpha}{nk} \big)^{(10k)^{7k}}$.  This hypothetical $k$-tuple must also be close to the $k$-tuple of true components.  We can output this hypothesis.  This completes the proof.
\end{proof}


==> extras2.tex <==
\section{Lower Bounds}
In this section, we show information-theoretic lower bounds on the number of samples required to identify a mixture of $k$ Mallows models under the condition that the components are separated from each other and from the uniform distribution by total variation distance at least $\mu$.  In particular, we show necessary dependence on $\mu^k$.  Our general method will be to exhibit two mixtures of Mallows models that are $ \approx \mu^k$ close in total variation distance.  The precise statement of our result is as follows.

\begin{theorem}\label{lowerBound1}
There exist two mixtures of at most $k$ Mallows models $M_1, \cdots ,M_a$ and $M_1', \cdots ,M_b'$ ($a,b \leq k$) with mixing weights $w_1, \cdots , w_a$ and $w_1' , \cdots , w_b'$ respectively, such that 
\begin{itemize}
\item[(a)] The total variation distance between any two of the components and between any component and the uniform distribution is at least $\mu$.
\item[(b)] $w_i,w_i' \geq \frac{1}{10 \cdot 2^k}$ for all $i$
\item[(c)] The total variation distance between the mixtures is at most $4(4\mu k)^{k-1}$
\end{itemize}
In particular, this shows that $\mu^k$ dependence is necessary for the sample complexity of our algorithms.
\end{theorem}


\begin{proof} We will first work with vectorizations of Mallows models and exhibit a linear combination with small $L^1$-norm and at the end we will use this linear combination to produce the two mixtures.



Set $\pi$ as the identity permutation on $[n]$ and consider $M_1(\phi_1, \pi), \cdots ,M_k(\phi_k,\pi)$ where $\phi_1 = \psi, \phi_2 = 2\psi, \cdots, \phi_k = k\psi$ for some $\psi$ that we will choose later.  Also define $F(\phi) = (1+\phi) \cdots (1+\phi+ \cdots + \phi^{n-1})$.  Now consider the linear combination
\[
v = \binom{k-1}{0} F(\phi_1)v(M_1) - \binom{k-1}{1}F(\phi_2)v(M_2) + \cdots + (-1)^{k-1}\binom{k-1}{k-1}F(\phi_k)v(M_k)
\]
\begin{claim}
$||v||_{L^1} \leq \frac{(2nk\psi)^{k-1}}{1-2nk\psi}$
\end{claim}
\begin{proof}
For a given permutation $\pi'$ that has $i$ inversions, the value of the above at the entry indexed by $\pi'$ is 
\[
\psi^i \sum_{j=0}^{k-1} (-1)^j\binom{k-1}{j} (j+1)^i
\]
which is $0$ when $i \leq k-2$ and is at most $(2k \psi)^i$ when $i \geq k-1$.  Now we show there are at most $n^i$ permutations with exactly $i$ inversions.  To do this we use induction.  The base case for $n=0$ is trivial.  Now for each permutation with exactly $i$ inversions (assume $i>0$), we correspond it to a permutation with exactly $i-1$ inversions by swapping the first two adjacent elements that are out of order.  Clearly at most $n$ permutations with $i$ inversions can correspond to the same permutation with $i-1$ inversions and this completes the induction.  Thus we can now bound 
\[
||v||_{L^1} \leq \sum_{i=k-1}^{\infty} (2nk\psi)^i \leq \frac{(2nk\psi)^{k-1}}{1-2nk\psi}
\]
\end{proof}

Assume $\mu <\frac{1}{100k^2}, n>100k^2$.  We now show that we can choose $\psi = \frac{2\mu}{n}$.  We calculate the probability of obtaining the identity permutation as a sample from $M_i$.  This is exactly 
\[
P_i(\pi) = \frac{1}{(1+i\psi) \cdots (1+ i\psi + \cdots + (i\psi)^{n-1})} = \frac{(1-i\psi)^{n-1}}{(1-(i\psi)^2) \cdots (1-(i\psi)^{n})}
\]
The numerator is $(1-\frac{2i\mu}{n})^{n-1} = ( (1-\frac{2i\mu}{n} )^{\frac{n}{2i\mu}} ) ^{2i\mu} (1-\frac{2i\mu}{n})^{-1} $.
We have
\[
\big(1-\frac{2i\mu}{n} \big)e^{-1} < \big(1-\frac{2i\mu}{n} \big)^{\frac{n}{2i\mu}} < e^{-1}
\]
Also $1-2i\mu < e^{-2i\mu} < 1-2i\mu + (4i^2\mu^2) < 1-(2i-0.1)\mu$.  Thus the numerator is between $1- 2i\mu$ and $\frac{1-(2i-0.1)\mu}{1-\frac{2i\mu}{n}} < 1-(2i-0.5)\mu$ for $n$ sufficiently large. The denominator is between $1$ and $1- \frac{(i\psi)^2}{1-i\psi}$.  Thus for $n$ sufficiently large, we can ensure that 
\[
1-2i\mu \leq P_i(\pi) \leq 1-(2i-1)\mu
\]
and this immediately gives us that that the total variation distance between any two of the $M_i$ is at least $\mu$.  It is also clear from the above that the total variation distance from the uniform distribution is at least $\mu$.  With the above choice of $\psi$, we have that $||v||_{L^1} \leq 2(4\mu k)^{k-1}$.  Now if the sum of the coefficients in $v$ is positive, add some constant to the coefficient of $v(M_2)$ so that the sum of the coefficients is zero.  If the sum is negative, add some constant to the coefficient of $v(M_1)$ so that the sum of the coefficients is zero. Regardless, adding this correction term will at most double the $L^1$ norm of $v$ since before adding this term, the $L^1$ norm of $v$ is at least absolute value of the sum of the coefficients.  Now consider two mixtures, one consisting of the positive terms of $v$ and the other consisting of the negative terms of $v$ with coefficients normalized so that the sum of the weights of both sides is $1$.  The minimum of the mixing weights on both sides is at most $\frac{1}{10 \cdot 2^k}$ (note $F(\phi_i) < \frac{1}{(1-\phi_i)^n} < 10$ for all $1 \leq i \leq k$). Also, the total variation distance between these two mixtures is at most $4(4\mu k)^{k-1}$.  This completes the proof. \end{proof}


